Putting Peer Prediction Under the Micro(economic)scope and Making Truth-telling Focal

Peer-prediction is a (meta-)mechanism which, given any proper scoring rule, produces a mechanism to elicit privately-held, non-verifiable information from self-interested agents. Formally, truth-telling is a strict Nash equilibrium of the mechanism. Unfortunately, there may be other equilibria as well (including uninformative equilibria where all players simply report the same fixed signal, regardless of their true signal) and, typically, the truth-telling equilibrium does not have the highest expected payoff. The main result of this paper is to show that, in the symmetric binary setting, by tweaking peer-prediction, in part by carefully selecting the proper scoring rule it is based on, we can make the truth-telling equilibrium focal---that is, truth-telling has higher expected payoff than any other equilibrium. Along the way, we prove the following: in the setting where agents receive binary signals we 1) classify all equilibria of the peer-prediction mechanism; 2) introduce a new technical tool for understanding scoring rules, which allows us to make truth-telling pay better than any other informative equilibrium; 3) leverage this tool to provide an optimal version of the previous result; that is, we optimize the gap between the expected payoff of truth-telling and other informative equilibria; and 4) show that with a slight modification to the peer prediction framework, we can, in general, make the truth-telling equilibrium focal---that is, truth-telling pays more than any other equilibrium (including the uninformative equilibria).

==> focal.tex <==


\gs{not sure where this goes}

%\gs{I am too tired to redo this now, but it does not seem right}
Recall, we use the term {\emph{focal}} to refer to an equilibrium with expected payoff strictly higher than that of any other symmetric Bayesian Nash equilibrium.
In this section, we prove that for almost any symmetric prior, there exists a strictly proper scoring rule such that truth-telling is the focal equilibrium of the peer prediction mechanism using that scoring rule.   We undertake this in two steps, distinguishing between two types of non-truthtelling equilibria of the peer prediction mechanism.  First we show how to choose the proper-scoring rule so that truth-telling is focal among the informative equilibrium.  Then, given those results, we show how to modify the payments so that the uninformative equilibria pay less, in expectation, than truth-telling.\\
For convenience, we denote $q^*(1) $ by $ q^* $.
\gs{better place?}
%%\gs{I am too tired to redo this now, but it does not seem right}
%Recall, we use the term {\emph{focal}} to refer to an equilibrium with strictly higher expected payoff than any other symmetric Bayesian Nash equilibrium.
%In this section, we prove the following results: (1) for almost any symmetric prior, there exists a strictly proper scoring rule such that truth-telling is the focal equilibrium of the peer prediction mechanism using that scoring rule, (2) for almost any symmetric prior, for a large family of strictly proper scoring rules, the scoring rule can be modified via an affine shift of its inputs so that truth-telling is the focal equilibrium of the peer prediction mechanism using that scoring rule, and (3) we show how to compute, for nearly any prior, the best strictly proper scoring rule, i.e.\ the scoring rule that, when used in the peer prediction mechanism, yields the largest possible gap between the payoff of truth telling and that of any other equilibrium.


\gs{end}



==> futurework.tex <==
Several open questions remain.  The first is to generalize this beyond binary signals.  One difficulty in handling this case is that the number of non-truthtelling equilibrium grows exponentially in the signal size.   Another question is whether these results can be extended to the Bayesian Truth Serum~\cite{prelec2004bayesian} or Robust Bayesian Truth Serum~\cite{witkowski2012robust} mechanisms (which have relaxed common prior assumptions).    

==> higher_dimension.tex <==

We consider the case in which instead of receiving one private bit $b_i \in \left\{0,1\right\}$, each player $i$ receives a private signal $\boldsymbol{\sigma_i}=(b_i^1,...,b_i^d) \in \left\{0,1\right\}^d$ where $d \geq 1$. Let us write $q_k(1|b)=P(b_j^k=1|b_i^k=b)$ for any pair of players $(i,j) \in [n]^2$ and any $k \in [d]$, and let $PS^k(p,q)$ be our 1-dimensional scoring rule for games in which $q_k(1|b)=q(1|b)$. Our peer prediction setting works as follows:
\begin{itemize}
\item Each agent $i \in [n]$ chooses a vector $\boldsymbol{\hat{b}_i}$ to report.
\item For every agent $i$, our algorithm chooses a bit $k \in [d]$ uniformely at random as well as a player $j$ uniformely at random among $1,..,i-1,i+1,...,n$, and pays agent $i$ $PS^k(\hat{b}_j^k,q_k(1|\hat{b}_i^k))$.
\end{itemize}

We denote the strategy of player $i$ by $ \boldsymbol{\theta_i}=(\theta_i^1,...,\theta_i^d)$, and we write $  \boldsymbol{\theta^k}=(\theta_1^k,...,\theta_n^k)$ the projection of the strategies of the players on bit $k$.

\begin{lemma}
$\boldsymbol{\theta}=(\theta^1,...,\theta^d)$ is an equilibrium strategy in the d-dimensional case if and only if $\forall k \in [d]$, $\boldsymbol{\theta^k}$ is an equilibrium strategy for the 1-dimensional game $G^k$ with $q(1|b)=q_k(1|b)$. 
\end{lemma}

\begin{proof}
Suppose $\boldsymbol{\theta}$ is a Nash equilibrium of the d-dimensional game, but there is $k$ such that $\boldsymbol{\theta^k}$ is not an equilibrium strategy for the 1-dimensional projection of the game on bit $k$. Therefore, there must exist a deviation $\tilde{\theta}^{k}_i$ for at least one player $i$ such that it increases his expected payoff: $u_i^k(\theta^k_1,...,\theta_i^k,...,\theta_n^k)< u_i^k(\theta^k_1,...,\tilde{\theta}_i^k,...,\theta_n^k)$, where $u_i^k$ is the payoff of player $i$ in the 1-dimensional game $G^k$ in which $q(1|b)=q_k(1|b)$. But now, if player $i$ plays $\boldsymbol{\tilde{\theta}_i}=(\theta_i^1,...,\tilde{\theta}_i^k,...,\theta_i^n)$ in the d-dimensional game, he gets payoff (we just condition on the bit we choose): 

\begin{align*}
 u_i(\boldsymbol{\theta_1},...,\boldsymbol{\tilde{\theta}_i},...,\boldsymbol{\theta_n})=\frac{1}{d}[\sum\limits_{l=1, l\neq k}^d u_i^l(\theta_1^l,...,\theta_n^l) +  u_i^k(\theta^k_1,...,\tilde{\theta}_i^k,...,\theta_n^k)]
\\ >\frac{1}{d}[\sum\limits_{l=1, l\neq k}^d u_i^l(\theta_1^l,...,\theta_n^l) +  u_i^k(\theta^k_1,...,\theta^k_i,...,\theta_n^k)] 
\\=\frac{1}{d} \sum\limits_{l=1}^d u_i^l(\theta_1^l,...,\theta_n^l)=u_i(\boldsymbol{\theta_1},...,\boldsymbol{\theta_n}).
\end{align*}
\\Therefore, player $i$ is better off by deviating from $\boldsymbol{\theta_i}$ to $\boldsymbol{\tilde{\theta}_i}$ while other players' strategies are fixed, meaning that $S$ cannot be a Nash equilibrium. Contradiction. This proves the forward implication. 
\\The backward implication follows from a similar argument: if $\boldsymbol{\theta^k}$ is an equilibrium strategy for all $k$, then it means that for all $i$, no deviation of player $i$ can improve $u_i^k(\boldsymbol{\theta^k})$ for any player $i$. But then, no deviation of player $i$ can improve $u_i(\boldsymbol{\theta})=\frac{1}{d} \sum\limits_{k=1}^d u_i(\boldsymbol{\theta^k})$ (as any deviation from $S$ by player $i$ is a deviation from one or several $\boldsymbol{\theta^k$}'s by player $i$), and $\boldsymbol{\theta}$ has to be an equilibrium strategy.
\end{proof}

\begin{lemma}
Let $\boldsymbol{\theta}=(\boldsymbol{\theta_1},...,\boldsymbol{\theta_d})$ be the highest paying-off equilibrium of the d-dimensional game. Then $\forall k \in [d]$, $\boldsymbol{\theta^k}$ is the highest paying-off equilibrium strategy for the 1-dimensional game $G^k$ with $q(1|b)=q_k(1|b)$. 
\end{lemma}

Note that as a direct consequence of lemma 1 and the nonexistence of symmetric equilibria in the 1-dimensional case \jz{This should be kept only if the proof of nonexistence of asymmetric eauilibria is right}, every equilibrium of the d-dimensional case must be symmetric. Therefore, the expected utilities of the players are identical and we now use $u$ instead of $u_i$.

\begin{proof}
Suppose this is not the case. Then there exists $k$ such that $\boldsymbol{\theta^k}$ is not the highest paying-off equilibrium of $G^k$; we know from lemma 1 that $\boldsymbol{\theta^k}$ is an equilibrium strategy for $G^k$, and therefore there must be an equilibrium $\tilde{\theta}^k$ for $G^k$ such that $u^k(\theta^k) < u^k(\tilde{\theta}^k)$. But now, let $\tilde{\boldsymbol{\theta}}=(\boldsymbol{\theta^1},...,\boldsymbol{\tilde{\theta}^k},...,\boldsymbol{\theta^d})$, we have:
\[
u(\boldsymbol{\tilde{\theta}})=\frac{1}{d}(\sum\limits_{l=1,l \neq k}^d u^l(\boldsymbol{\tilde{\theta}_l})+u^k(\boldsymbol{\tilde{\theta}_k})) >\frac{1}{d} \sum\limits_{l=1}^d u^l(\boldsymbol{\theta_l}) = u(\boldsymbol{\theta})
\]
and $\tilde{\theta}$ is an equilibrium by lemma 1. So $\theta$ is not the highest paying-off equilibrium, contradiction.
\end{proof}

\begin{corollary}
If for all $k$, $PS^k(p,q)$ is a one-dimensional scoring rule such that the all-truth equilibrium is the unique highest paying-off equilibrium of $G^k$, then the all-truth equilibrium is the highest paying-off equilibrium in the d-dimensional game.
\end{corollary}

\begin{proof}
Let $S$ be the  highest paying-off equilibrium of the d-dimensional game, it follows that for all $k$, $\boldsymbol{\theta^k}$ is the  highest paying-off equilibrium of $G^k$; therefore, $\boldsymbol{\theta^k}$ is the all-truth equilibrium. It immediately follows that $S$ is the all-truth equilibrium of the d-dimensional game. 
\end{proof}

By using the same argument as in the proof of the lemma, i.e. the fact that the expected payoff of of the d-dimensional case is simply a convex combination of the 1-dimensional payoffs, it is straightforward to see that the gap between the truthful equilibrium and the second highest paying-off equilibrium is maximized when the gap of the projection on bit $k$ is maximized for every $k$, and any bound on the maiximizer that holds in the 1-dimensional case similarly holds in the d-dimensional case. Therefore, all of our unidimensional optimization statements apply to this more general case.

\jz{I did not include an optimization statement when I first wrote the proof, but it's really straightforward: we just need to apply the same idea as here. It's probably something that we can mention in a few sentences? I was thinking of something in the lines of "by the same argument, it is straightforward to see that the gap between the truthful equilibrium and the second highest paying-off equilibrium is maximized when the gap of the projection on bit $k$ is maximized for every $k$, and any bound that holds in the 1-dimensional case similarly holds in the d-dimensional case"}


==> optimization-saved.tex <==
\ifnum\fullversion=1

%For any two real numbers $ l<u $, $ PF\in[l,u] $ means that $ \min_{i,j=0,1}PF(i,j)=l,\max_{i,j=0,1}PF(i,j)=u $
%Let $ %\mathcal{U}=\{PF|\min_{i,j=0,1}PF(i,j)=0,\max_{i,j=0,1}PF(i,j %)=1\} $
%\end{definition}
%For positively correlated Q, let $ \alleq_{Q}(PF) $ be the set of equilibria under payoff function $ PF $. Let $$ \Delta_Q(PF)=[\nu^{PF}(\tru)- \max_{\theta\in \alleq_{Q}(PF)/\{\tru,\zer,\one\}} \nu^{PF}(\theta)] $$ be the gap between truth-telling's payoff and the maximal payoff of all other informative equilibria when $ PF\in \mathcal{U} $. For any given symmetric and positively correlated $ Q $, we would like to
%\begin{enumerate}
%\item solve $$ %\Delta^*(Q)=\sup_{PF\in\mathcal{U}}\Delta_{Q}(PF)  $$
%\item either find $ PF^*\in \mathcal{U} $ such that $ \Delta_Q(PF^*)=\Delta^*(Q) $ or; if such $ PF^* $ doesn't exist, then $ \forall \epsilon>0 $, find $ PF^*(\epsilon) $ such that $ \Delta_Q(PF^*(\epsilon))>\Delta^*(Q)-\epsilon $. We call a prior $ Q $ attainable prior if $ \exists PF^* $ such that $ \Delta_Q(PF^*)=\Delta^*(Q) $; otherwise we call the prior unttainable prior.
%\end{enumerate}

%We fulfill these goals and find the region where prior is attainable.

%We will divide the positively correlated priors into three regions which correspond to three payoff functions which (almost) attain the optimal gap $ \Delta^*(Q) $. These three regions are(See figure~\ref{fig:attainableprior}):
%\begin{figure}
%\centering
%\includegraphics[scale=0.3]{attainableprior.jpg}
%\caption{The triangle is an area where the prior is positively correlated($ q(1|1)>q(1|0) $) and $ q(1|1)>q(0|0) $. The case of $ q(1|1)<q(0|0) $ is analogous. The prior is attainable in $ R_1 $ and $ R_2 $ while the prior is unattainable in $ R_3 $. }
%\label{fig:attainableprior}
%\end{figure}
Now we will restate Theorem~\ref{opt_thm} in detail and prove it.

\begin{definition}\label{attainable prior}

\begin{align*}
R_1=&\{q(0|0)\leq q(1|0)\}\cup\\
&\{q(0|0)>q(1|0) \wedge q^*_{a,o}>q(0|0)\wedge \Delta^*_a(Q)\geq \Delta^*_b(Q) \}\\
R_2=& \{q(0|0)>q(1|0) \wedge q^*_{a,o}>q(0|0)\wedge \Delta^*_a(Q)< \Delta^*_b(Q) \}\cup\\
&\{ q(0|0)>q(1|0) \wedge q^*_{a,o}\leq q(0|0)\wedge \xi(k^{sup}_a(q(0|0)),q(0|0))\leq \Delta^*_b(Q) \}\\
R_3 =& \{ q(0|0)>q(1|0) \wedge q^*_{a,o}\leq q(0|0)\wedge \xi(k^{sup}_a(q(0|0)),q(0|0))> \Delta^*_b(Q) \}\\
\end{align*}
%$$ R_1=\{q(0|0)\leq q(1|0)\}\cup \{q(0|0)>q(1|0) \& q_{a,o}>q(0|0)\& \Delta^*_a(Q)\geq \Delta^*_b(Q) \} $$
%$$ R_2 = \{q(0|0)>q(1|0) \& q_{a,o}>q(0|0)\& \Delta^*_a(Q)< \Delta^*_b(Q) \}\cup\{ q(0|0)>q(1|0) \& q_{a,o}\leq q(0|0)\& \iota(q(0|0))\leq \Delta^*_b(Q) \} $$
%$$ R_3 = \{ q(0|0)>q(1|0) \& q_{a,o}\leq q(0|0)\& \iota_a(q(0|0))> \Delta^*_b(Q) \} $$
where
$ q^*_{a,o}=\frac{q(1|0)q(1|1)-\sqrt{q(1|0)q(0|1)q(0|0)q(1|1)}}{q(1|1)-q(0|0)} $,\\
$ \Delta^*_a(Q)=\frac{q(0|1)(q(0|0)q(1|0)-\sqrt{q(0|0)q(1|0)q(0|1)q(1|1)})(\sqrt{q(0|0)q(1|0)q(0|1)q(1|1)}-q(0|1)q(1|1))}{(q(0|1)+q(1|0)q(1|1)(q(1|1)-q(0|0))(\sqrt{q(0|0)q(1|0)q(0|1)q(1|1)}+q(1|1)-q(0|0)-q(1|0)q(1|1))} $,\\
$ \Delta^*_b(Q)=\frac{(q(1|1)-q(0|0))(q(0|0)q(1|0)(q(1|1)-q(0|1))-\sqrt{q(0|0)q(1|0)(q(1|1)-q(1|0))(q(1|1)-q(0|0))})}{(q(1|0)+q(0|1))q(1|0)q(1|1)q(0|0)} $, \\
$ \xi(k^{sup}_a(q(0|0)),q(0|0))=\min\{\iota_a(q(0|0)),\kappa_a(q(0|0))\} $\\
where $ \iota_a(q(0|0))=\frac{q(0|1)}{q(1|0)+q(0|1)} \frac{q(1|0)(q(1|1)-q(0|0))( q(0|0)-q(1|0))}{ q(0|0)((q(1|1)-q(0|0))q(0|0)-q(1|0)q(1|1)) } $,\\
$ \kappa_a(q(0|0))=\frac{q(0|1)}{q(1|0)+q(0|1)}\frac{(q(1|1)-q(0|0))(q(0|0)-q(1|0))}{q(1|1) (1-q(0|0))} $\\

\end{definition}
$ R_1 $ and $ R_2 $ contain \textit{attainable priors} while $ R_3 $ contain \textit{unattainable priors}.
\smallskip

The optimization theorem we will show is:

\begin{theorem}[optimization theorem]
For any positively correlated prior Q with $ q(1|0)\neq q(0|1) $ and with $ q(1|1)>q(0|0) $(the result for $ q(0|0)<q(1|1) $ is analogous),
\begin{description}
\item[1]If $ Q\in R_1 $: $\Delta_{Q}(\mathcal{M}_1(Q))=\Delta^*(Q)$\\

\item[2]If $ Q\in R_2 $: $\Delta_{Q}(\mathcal{M}_2(Q))=\Delta^*(Q)$\\

\item[3]If $ Q\in R_3 $: $ \lim_{\epsilon\rightarrow 0^{+}}\Delta_{Q}(\mathcal{M}_3(Q,\epsilon))=\Delta^*(Q) $\\

\end{description}
where

$\mathcal{M}_1(Q) = \left( \begin{array}{ccc}
\zeta(Q) & & 0\\
 & & \\
0 & & 1\\
\end{array} \right)$, $\mathcal{M}_2(Q) =\left( \begin{array}{ccc}
1 & & 0\\
 & & \\
0 & & \eta(Q)\\
\end{array} \right) $, $\mathcal{M}_3(Q,\epsilon) =\left( \begin{array}{ccc}
\zeta(Q,\epsilon) & & \delta(Q,\epsilon)\\
 & & \\
0 & & 1\\
\end{array} \right) $ and\\
$  \zeta(Q)=\sqrt{\frac{q(0|0) q(0|1)}{q(1|0) q(1|1)}}   $, $  \eta(Q)=\frac{1}{q(1|1)}(\sqrt{\frac{(q(1|1)-q(1|0))(q(1|1)-q(0|0))}{q(0|0)q(1|0)}}-q(0|1))   $,\\
$\zeta(Q,\epsilon)=\frac{q(0|0) q(0|1)}{q(0|0) q(0|1) q(0|0)+\epsilon+q(1|0) (q(1|1)-q(1|1)
   q(0|0)+\epsilon)}$,\\
$\delta(Q,\epsilon)=\frac{q(1|0) q(1|1) (q(0|0)+\epsilon-1)^2-q(0|0) q(0|1) q(0|0)+\epsilon^2}{q(0|0)+\epsilon (q(1|0)
      q(1|1) (q(0|0)+\epsilon-1)-q(0|0) q(0|1) q(0|0)+\epsilon)}$\\




\end{theorem}


\begin{definition}\label{normalization}
We define $ \mathcal{N}(\cdot) $ as a normalization function and $$ \mathcal{N}(PF)=\frac{PF-\min_{i,j}PF(i,j)}{\max_{i,j}PF(i,j)-\min_{i,j}PF(i,j)}. $$ It is clear that $ \mathcal{N}(PF)\in \mathcal{U} .$
\end{definition}

After we define the normalization function, we have $$ \sup_{PF\in\mathcal{U}}\Delta_{Q}(PF)=\sup_{PF}\Delta_{Q}(\mathcal{N}(PF)).$$

\begin{definition}
We define $ G(\cdot) $ as a function to map $ \{\alpha,\beta,q^*,\gamma\} $ to a payoff function $ PF $ such that $ \forall i,j=0,1, PF(i,j)=\ell(i,j) $ and $ \ell(x,1)=\alpha (x-q^*)+\gamma $ and $ \ell(x,0)=\beta (x-q^*)+\gamma $.
\end{definition}
Notice that in the $ R_{\tru} $ region, the slope of the contours is $$k=-\frac{\beta q(0|1)}{\alpha q(1|0)},$$ so $ \beta $ can be represented as $ -k \alpha\frac{ q(1|0)}{q(0|1)} $.

\katrina{Where did we establish the definition of $q^*$?}

\paragraph{Proof Overview for Theorem~\ref{opt_thm}} We will show three lemmas to prove Theorem~\ref{opt_thm}. In the first lemma (Lemma~\ref{optgoal}), we show that the gap $ \Delta_Q(\mathcal{N}(PF)) $ we want to optimize only depends on the value of $ q^* $ and the slope $ k $ of contours in the $ R_{\tru} $ region. Let $$ \xi(k,q^*)=\Delta_Q(\mathcal{N}(PF)). $$ The goal is to solve $\sup_{k,q^*}\xi(k,q^*)$; notice that
\begin{align*}
\sup_{k,q^*}\xi(k,q^*)&=\sup_{q^*}\sup_{k}\xi(k,q^*).\\
\end{align*}
In the second lemma (Lemma~\ref{main_Lemma}), we  show for any $ q(1|0)<q^*<q(1|1) $, there exists $ k^{sup}(q^*) $ such that $$ \xi(k^{sup}(q^*),q^*)=\sup_k \xi(k,q^*).$$ In the third lemma(Lemma~\ref{qstarvalue}), we will solve $$ \sup_{q^*}\xi(k^{sup}(q^*),q^*).$$
Combining these three lemmas, Theorem~\ref{opt_thm} will follow.


\begin{lemma}\label{optgoal}
For any $ PF=G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma) $, $$ \Delta_Q(\mathcal{N}(PF))=\nu^{\mathcal{N}(PF)}(\tru)- \max_{\theta\in \alleq_Q(\mathcal{N}(PF))/\{\tru,\zer,\one\}} \nu^{\mathcal{N}(PF)}(\theta) $$ only depends on $ q^* $ and $ k $ which is the slope of contours in $ R_{\tru} $.
Let $$ \xi(k,q^*)=\Delta_Q(\mathcal{N}(PF)). $$
\end{lemma}

\begin{lemma}\label{kvalue}
There exists $ k^{sup}(q^*) $ such that $$ \xi(k^{sup}(q^*),q^*)=\sup_k \xi(k,q^*) $$
$$ k^{sup}(q^*)=\left\{
\begin{array}{rcl}
k^{sup}_a(q^*)       &      & {q^*>q(0|0)}\\
       &      &       \\
k^{sup}_b(q^*)    &      & {q^*\leq q(0|0)}
\end{array} \right. $$
Where $$ k^{sup}_a(q^*)=\frac{f(\tru\one)_y-f(\tru\zer)_y}{f(\tru\one)_x-f(\tru\zer)_x} $$ $$ k^{sup}_b(q^*)=\frac{f(\tru\one)_y-f(\fal_y)}{f(\tru\one)_x-f(\fal_x)} $$ and $ f $ is translation map (see description~\ref{translationmap}).
\end{lemma}

\begin{figure}
\centering
\includegraphics[scale=0.45]{Unattainablecase.jpg}
\caption{The x axis is $ q^* $, the y axis is the gap we would like to optimize. This figure is an illustration of the results in Lemma~\ref{qstarvalue}. }
\label{fig:Unattainablecase}
\end{figure}


\begin{lemma}\label{qstarvalue}
$ \xi(k^{sup}_a(q^*),q^*) $ is first increasing and then decreasing in the $ [q(1|0), q(1|1)] $ region; $ \xi(k^{sup}_b(q^*),q^*) $ is first increasing and then decreasing in the $ [q(1|0), q(0|0)] $ region. If we denote $ \sup_{q^*}\xi(k^{sup}_a(q^*),q^*) $ by $ \Delta^*_a(Q) $; denote $ \sup_{q^*}\xi(k^{sup}_b(q^*),q^*) $ by $ \Delta^*_b(Q)$, then there exists $ q(1|0)<q^*_{a,o}<q(1|1) $, $ q(1|0)<q^*_{b,o}<q(0|0) $ such that $ \forall I\in\{a,b\} $ $$ \xi(k^{sup}_I(q^*_{I,o}),q^*_{I,o})=\Delta_I^*(Q)$$ and $ NG(k^{sup}_I(q^*_{I,o}),q^*_{I,o}) $ is a normalized payoff function and let $ PF^* $ denote it. We have $$ PF^*(0,1)=PF^*(1,0)=0.$$
Moreover, $$NG(k^{sup}_a(q^*_{a,o}),q^*_{a,o})= \mathcal{M}_1(Q),$$
$$NG(k^{sup}_b(q^*_{b,o}),q^*_{b,o})=\mathcal{M}_2(Q),$$
and when $ q^*_{a,o} \leq q(0|0) $, $ \epsilon>0 $, $$NG(k^{sup}_a(q(0|0)+\epsilon),q(0|0)+\epsilon)=\mathcal{M}_3(Q,\epsilon).$$
\end{lemma}


We defer the proofs of these lemmas, and first show how Theorem~\ref{opt_thm} follows from them.

\begin{figure}
\centering
\includegraphics[scale=0.5]{Unattainablecase2.jpg}
\caption{Here is the case: $ q(0|0)>q^*_{a,o} $ and $ \sup_{k,q^*}\xi(k,q^*)=\lim_{\epsilon\rightarrow 0^{+}}\xi(k^{sup}_a(q(0|0)+\epsilon),q(0|0)+\epsilon) $, since we can not obtain this supremum, this prior here is unattainable.  }
\label{fig:Unattainablecase2}
\end{figure}

\begin{proof}[of Theorem~\ref{opt_thm}]

Based on Lemma~\ref{kvalue} and Lemma~\ref{qstarvalue}, we have
\begin{align*}
\sup_{k,q^*}\xi(k,q^*)
&=\max\{\sup_{q^*\leq q(0|0)}\sup_{k}\xi(k,q^*),\sup_{q^*> q(0|0)}\sup_{k}\xi(k,q^*)\}\\
&=\max\{\sup_{q^*\leq q(0|0)}\xi(k^{sup}_b(q^*),q^*),\sup_{q^*> q(0|0)}\xi(k^{sup}_a(q^*),q^*)\}\\
\end{align*}
\begin{enumerate}
\item If $ q^*_{a,o}>q(0|0) $, then \begin{align*}
\sup_{k,q^*}\xi(k,q^*)&= \max\{\xi(k^{sup}_b(q^*_{b,o}),q^*_{b,o}),\xi(k^{sup}_a(q^*_{a,o}),q^*_{a,o})\}\\
\end{align*}
Since $ \Delta^*_a(Q)=\xi(k^{sup}_a(q^*_{a,o}),q^*_{a,o}) $, $ \Delta^*_b(Q)=\xi(k^{sup}_b(q^*_{b,o}),q^*_{b,o}) $  Then
$$ \sup_{PF\in\mathcal{U}}\Delta_Q(PF)=\sup_{k,q^*}\xi(k,q^*)=
\begin{cases}
\Delta_Q(\mathcal{M}(Q_1)) \  if\  \Delta^*_b(Q)<\Delta^*_a(Q)\\
\Delta_Q(\mathcal{M}(Q_2)) \  if\ \Delta^*_a(Q)\leq\Delta^*_b(Q)\\
\end{cases} $$
\item If $ q^*_{a,o}\leq q(0|0) $, then  \begin{align*}
\sup_{k,q^*}\xi(k,q^*)&= \max\{\xi(k^{sup}_b(q^*_{b,o}),q^*_{b,o}),\xi(k^{sup}_a(q(0|0)),q(0|0))\}\\
\end{align*}
If $ \xi(k^{sup}_a(q(0|0)),q(0|0))\leq\xi(k^{sup}_b(q^*_{b,o}),q^*_{b,o}) $, we have $$ \sup_{PF\in\mathcal{U}}\Delta_Q(PF)=\Delta_Q(\mathcal{M}_2(Q)) $$
If $ \xi(k^{sup}_b(q^*_{b,o}),q^*_{b,o})<\xi(k^{sup}_a(q(0|0)),q(0|0)) $(See Figure\ref{fig:Unattainablecase2}), then
\begin{align*}
\lim_{\epsilon\rightarrow 0^{+}}\xi(k^{sup}_a(q(0|0)+\epsilon),q(0|0)+\epsilon)=\sup_{k,q^*}\xi(k,q^*)
\end{align*}
Then let $ \mathcal{M}_3(Q,\epsilon)=NG(k^{sup}_a(q(0|0)+\epsilon),q(0|0)+\epsilon)) $, $$\sup_{PF\in\mathcal{U}}\Delta_Q(PF)=\lim_{\epsilon\rightarrow 0^{+}}\Delta_Q(\mathcal{M}_3(Q,\epsilon))$$
\end{enumerate}
\end{proof}



\subsection{Proof for Lemma~\ref{optgoal}}\label{sec:optgoal}

\begin{lemma}\label{kqstar}
If $ \alpha>0 $, $ \mathcal{N}(G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma)) $ only depends on $ k,q^* $, we denote $ \mathcal{N}(G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma)) $ by $$  NG(k,q^*) $$ Moreover, $$NG(k,q^*)=\left(\begin{array}{ccc}
\hat{\alpha}(k,q^*)(1-q^*)+\hat{\gamma}(k,q^*) & & -\hat{\alpha}(k,q^*)\frac{k q(1|0)}{q(0|1)} (1-q^*)+\hat{\gamma}(k,q^*)\\
\hat{\alpha}(k,q^*)(-q^*)+\hat{\gamma}(k,q^*) & &-\hat{\alpha}(k,q^*)\frac{k q(1|0)}{q(0|1)} (-q^*)+\hat{\gamma}(k,q^*) \\
\end{array}\right)$$ where $$\hat{\alpha}(k,q^*)=\frac{1}{\max_{i,j}\frac{PF(i,j)-\gamma}{\alpha}-\min_{i,j}\frac{PF(i,j)-\gamma}{\alpha}}$$ $$ \hat{\gamma}(k,q^*)=-\frac{\min_{i,j}\frac{PF(i,j)-\gamma}{\alpha}}{\hat{\alpha}(k,q^*)} $$
\end{lemma}
\begin{proof}[of Lemma~\ref{kqstar}]
Let $ PF $ be $ G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma) $, we have $ PF(1,1)=\alpha(1-q^*)+\gamma $, $ PF(1,0)=\beta(1-q^*)+\gamma $, $ PF(0,1)=\alpha(-q^*)+\gamma $, $ PF(0,0)=\beta(-q^*)+\gamma $ where $ \beta=-\frac{k \alpha q(1|0)}{q(0|1)} $
\begin{align*}
\mathcal{N}(G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma))=&\frac{PF-\min_{i,j}PF(i,j)}{\max_{i,j}PF(i,j)-\min_{i,j}PF(i,j)}\\
=&\frac{\frac{PF-\gamma}{\alpha}-\min_{i,j}\frac{PF-\gamma}{\alpha}(i,j)}{\max_{i,j}\frac{PF-\gamma}{\alpha}(i,j)-\min_{i,j}\frac{PF-\gamma}{\alpha}(i,j)}\\
\end{align*}
Since $ \frac{PF-\gamma}{\alpha} $ only depends on $ k,q^* $, the Lemma follows.
\end{proof}
\begin{remark}\label{normpayoffkqstar}
Based on Lemma~\ref{kqstar}, notice that for $ PF=G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma) $, $$\mathcal{N}(PF)=G'(k,q^*,\hat{\alpha}(k,q^*),\hat{\gamma}(k,q^*))$$ so nomalize payoff function won't change equilibria and the slope of the contours in the $ R_{\tru} $ region.
\end{remark}

\begin{proof}[of Lemma~\ref{optgoal}]
Since we only consider $ PF $ that making truth-telling focal, then $ \alpha>0 $, based on Remark~\ref{normpayoffkqstar}, we have $$ \alleq_Q(\mathcal{N}(PF))=\alleq_Q(\mathcal{N}(PF))=\alleq_Q(q^*) $$ and $$ \Delta_Q(\mathcal{N}(PF))=\Delta_Q(NG(k,q^*)) $$ then the lemma follows
\end{proof}



\subsection{Proof for Lemma~\ref{kvalue}}\label{sec:kvalue}

\begin{proof}[of Lemma~\ref{kvalue}]
We show this Lemma in two cases, \\
(1) If $ \max\{q(0|0),q(1|0)\}<q^*<q(1|1) $:\\
Based on Lemma~\ref{main_Lemma} and Corollary~\ref{the slope of contours}, there will be seven equilibria, and $$ \frac{q(0|1)}{q(0|0)}=\frac{f(\tru\one)_y-f(\tru)_y}{f(\tru\one)_x-f(\tru)_x}<k<\frac{f(\tru\zer)_y-f(\tru)_y}{f(\tru\zer)_x-f(\tru)_x}=\frac{q(1|1)}{q(1|0)} $$ if $ \tru $ is focal.
Also $$ \max_{\theta\in \alleq_Q(PF)/\{\tru,\zer,\one\}} \nu^{PF}(\theta)=\max\{\nu^{PF}(\tru \one),\nu^{PF}(\tru \zer)\} $$ So
\begin{align*}
 &\sup_{PF} [\nu^{\mathcal{N}(PF)}(\tru)- \max_{\theta\in \alleq/\{\tru,\zer,\one\}} \nu^{\mathcal{N}(PF)}(\theta)]\\
 =
 &\sup_{PF} [\min\{\nu^{\mathcal{N}(PF)}(\tru)-\nu^{\mathcal{N}(PF)}(\tru \one),\nu^{\mathcal{N}(PF)}(\tru)-\nu^{\mathcal{N}(PF)}(\tru \zer)\}]\\
\end{align*}
Since $ q^* $ is given, let $$ \phi^{q^*}(k) = \nu^{\mathcal{N}(PF)}(\tru)-\nu^{\mathcal{N}(PF)}(\tru \one)$$
$$ \psi^{q^*}(k) = \nu^{\mathcal{N}(PF)}(\tru)-\nu^{\mathcal{N}(PF)}(\tru \zer)$$
We have $$ \xi(k,q^*)=\min\{\phi^{q^*}(k),\psi^{q^*}(k)\} $$ We will show $ \phi^{q^*}(k) $ is increasing while $ \psi^{q^*}(k) $ is decreasing when $ \frac{q(0|1)}{q(0|0)}<k<\frac{q(1|1)}{q(1|0)} $. Then we can see when $ \phi^{q^*}(k)=\psi^{q^*}(k) $, $ \xi(k,q^*) $ gets maximum which means $$ \phi^{q^*}(k^{sup}_a(q^*))=\psi^{q^*}(k^{sup}_a(q^*)) $$  $$ \Rightarrow \nu^{\mathcal{N}(PF)}(\tru\one)=\nu^{\mathcal{N}(PF)}(\tru\zer) $$ $$ \Rightarrow k^{sup}_a(q^*)=\frac{f(\tru\one)_y-f(\tru\zer)_y}{f(\tru\one)_x-f(\tru\zer)_x} $$
Now we begin to show $ \phi^{q^*}(k) $ is increasing while $ \psi^{q^*}(k) $ is decreasing:\\
Since $$ \frac{q(0|1)}{q(0|0)}< k <\frac{q(1|1)}{q(1|0)}  $$
we can see
\begin{align*}
 PF(1,1)-PF(0,0)&=\ell(1,1)-\ell(0,0)\\
 &=\alpha(1-\frac{(q(0|1)+k q(1|0)) q^*}{q(0|1)})\\
 &<\alpha(1-\frac{(q(0|1)+\frac{q(0|1)}{q(0|0)} q(1|0)) q^*}{q(0|1)})\\
 &=\alpha (1-\frac{q^*}{q(0|0)})\\
 &<0
\end{align*}
So we can see $$ \max_{i,j=0,1}PF(i,j))=PF(0,0)=\ell(0,0) $$
Based on Lemma~\ref{normpayoffkqstar},
$$NG(k,q^*)=\left(\begin{array}{ccc}
\hat{\alpha}(k,q^*)(1-q^*)+\hat{\gamma}(k,q^*) & & -\hat{\alpha}(k,q^*)\frac{k q(1|0)}{q(0|1)} (1-q^*)+\hat{\gamma}(k,q^*)\\
\hat{\alpha}(k,q^*)(-q^*)+\hat{\gamma}(k,q^*) & &-\hat{\alpha}(k,q^*)\frac{k q(1|0)}{q(0|1)} (-q^*)+\hat{\gamma}(k,q^*) \\
\end{array}\right)$$ where
\begin{align*}
\frac{1}{\hat{\alpha}(k,q^*)}&=\max_{i,j}\frac{PF(i,j)-\gamma}{\alpha}-\min_{i,j}\frac{PF(i,j)-\gamma}{\alpha}\\
&=\frac{PF(0,0)-\gamma}{\alpha}-\min\{ \frac{PF(0,1)-\gamma}{\alpha},\frac{PF(1,0)-\gamma}{\alpha} \}\\
&=-\frac{kq(1|0)}{q(0|1)}(-q^*)-\min\{(-q^*,-\frac{kq(1|0)}{q(0|1)}(1-q^*)\}\\
&=\max\{(1+\frac{ k q(1|0)}{q(0|1)}) q^*,\frac{ k q(1|0)}{q(0|1)} \}\\
\end{align*}

Since the two linear functions $ \mathcal{N}(PF) $ represents are $ \ell^{\mathcal{N}(PF)}(y,1)=\hat{\alpha}(k,q^*)(y-q*)+\hat{\gamma}(k,q^*) $ and $ \ell^{\mathcal{N}(PF)}(x,0)=-\hat{\alpha}(k,q^*)\frac{k q(1|0)}{q(0|1)} (x-q^*)+\hat{\gamma}(k,q^*) $ and the expected payoff of points $ (x,y) $ in the $ R_{\tru} $ region is $$\nu^{\mathcal{N}(PF)}((x,y))= q(0)\ell^{\mathcal{N}(PF)}(x,0)+q(1)\ell^{\mathcal{N}(PF)}(y,1) $$ we have

\begin{align*}
\phi^{q^*}(k)&=\nu^{\mathcal{N}(PF)}(\tru)-\nu^{\mathcal{N}(PF)}(\tru \one)\\
%&=\frac{\nu^{PF}(\tru)-\nu^{PF}(\tru \one)}{\max\{(\alpha+\frac{\alpha k q(1|0)}{q(0|1)}) q^*,\frac{\alpha k q(1|0)}{q(0|1)} \}}\\
&=\hat{\alpha}(k,q^*) (-q(0)\frac{ k q(1|0)}{q(0|1)} (f(\tru)_x-f(\tru\one)_x)+q(1) (f(\tru)_y-f(\tru\one)_y))\\
%&=(\frac{q(0|1)}{q(0|1)+q(1|0)} \frac{-\alpha k q(1|0)}{q(0|1)} (\tru_x-\tru\one_x) + \frac{q(1|0)}{q(0|1)+q(1|0)} \alpha (\tru_y-\tru\one_y))/(\max\{(\alpha+\frac{\alpha k q(1|0)}{q(0|1)}) q^*,\frac{\alpha k q(1|0)}{q(0|1)} \})\\
%&=\frac{q(1|0)\alpha (\tru\one_x - \tru_x)}{q(0|1)+q(1|0)}(k-\frac{\tru_y-\tru\one_y}{\tru_x - \tru\one_x})/(\max\{(\alpha+\frac{\alpha k q(1|0)}{q(0|1)}) q^*,\frac{\alpha k q(1|0)}{q(0|1)} \})\\
%&=\frac{q(1|0) (\tru\one_x - \tru_x)}{q(0|1)+q(1|0)}(k-\frac{q(0|1)}{q(0|0)})/(\max\{(1+\frac{ k q(1|0)}{q(0|1)}) q^*,\frac{ k q(1|0)}{q(0|1)} \})\\
&=\frac{q(1|0) (q^* - q(1|0))}{q(0|1)+q(1|0)}(k-\frac{q(0|1)}{q(0|0)})/(\max\{(1+\frac{ k q(1|0)}{q(0|1)}) q^*,\frac{ k q(1|0)}{q(0|1)} \})\\
&=\frac{q(1|0) (q^* - q(1|0))}{q(0|1)+q(1|0)} \min\{ \frac{q(0|1)}{q^* q(1|0)} (1-\frac{\frac{q(0|1)}{q(0|0)q(1|0)}}{k+\frac{q(0|1)}{q(1|0)}}) , \frac{q(0|1)}{q(1|0)}-\frac{1}{k}\frac{q(0|1)^2}{q(0|0)q(1|0)} \}
\end{align*}
We can see $ \phi^{q^*}(k) $ is increasing since the for any two increasing functions $ f_1,f_2 $, $ \min\{f_1,f_2\} $ is still a increasing function.\\
Similarly, we replace $ \tru\one $ with $ \tru\zer $
\begin{align*}
&\psi^{q^*}(k)\\
=&\frac{q(1|0) (f(\tru)_x - f(\tru\zer)_x)}{q(0|1)+q(1|0)}(\frac{q(1|1)}{q(1|0)}-k)/(\max\{(1+\frac{ k q(1|0)}{q(0|1)}) q^*,\frac{ k q(1|0)}{q(0|1)} \})\\
\end{align*}
We can see $ \psi^{q^*}(k) $ is decreasing based on similar reason.\\

(2) If $ q(1|0)<q^*< q(0|0) $:\\

Based on Lemma~\ref{main_Lemma}, there will be nine or eight equilibria, and $$ \frac{q(0|1)}{q(0|0)}=\frac{f(\tru\one)_y-f(\tru)_y}{f(\tru\one)_x-f(\tru)_x}<k<\frac{f(\fal)_y-f(\tru)_y}{f(\fal)_x-f(\tru)_x}=\frac{(q(0|1)) (1-q^*)}{q(1|0)q^*} $$ if $ \tru $ is focal.
we can see
\begin{align*}
 PF(1,1)-PF(0,0)&=\ell(1,1)-\ell(0,0)\\
 &=\alpha(1-\frac{(q(0|1)+k q(1|0)) q^*}{q(0|1)})\\
 &>\alpha(1-\frac{(q(0|1)+\frac{(q(0|1)) (1-q^*)}{q(1|0)q^*}  q(1|0)) q^*}{q(0|1)})\\
 &=0
\end{align*}


Then the proof is similar with the previous case, we only need to relace $ f(\tru\zer) $ with $ f(\fal) $ $$ \phi^{q^*}(k^{sup}_b(q^*))=\psi^{q^*}(k^{sup}_b(q^*)) $$  $$ \Rightarrow \nu^{\mathcal{N}(PF)}(\tru\one)=\nu^{\mathcal{N}(PF)}(\fal) $$ $$ \Rightarrow k^{sup}_b(q^*)=\frac{f(\tru\one)_y-f(\fal)_y}{f(\tru\one)_x-f(\fal)_x} $$ \end{proof}


\subsection{Proof for Lemma~\ref{qstarvalue}}\label{sec:qstarvalue}

\begin{proof}[of Lemma~\ref{qstarvalue}]
Figure~\ref{fig:Unattainablecase} gives an illustration of the proof. We will show $$ \xi((k^{sup}_I(q^*),q^*)=\min\{\kappa_I(q^*),\iota_I(q^*) \} $$ and both $ \kappa_I(q^*) $ and $ \iota_I(q^*) $ are firstly increasing and then decreasing. Let $ q^*_{stat,\kappa} $ and $ q^*_{stat,\iota} $ be the stationary points of $ \kappa_I(q^*) $ and $ \iota_I(q^*) $. We will show $$ \max_{q^*}\kappa_I(q^*)=\max_{q^*}\iota_I(q^*) $$ Once we know it, we will use the property to prove there exists a point $ q^*_o $ between $ q^*_{stat,\kappa} $ and $ q^*_{stat,\iota} $ such that $$ \kappa_I(q^*_o)=\iota_I(q^*_o) $$ and $$ \xi(k^{sup}_I(q^*_o),q^*_o)=\sup_{q^*}\xi(k^{sup}_I(q^*),q^*)$$ and
$$ NG(k^{sup}_I(q^*_{o}),q^*_{o})(0,1)=NG(k^{sup}_I(q^*_{o}),q^*_{o})(1,0) $$
Now assuming we know $$ \max_{q^*}\kappa_I(q^*)=\max_{q^*}\iota_I(q^*) $$ we begin to prove there exists a point $ q^*_o $ between $ q^*_{stat,\kappa} $ and $ q^*_{stat,\iota} $ such that $$ \kappa_I(q^*_o)=\iota_I(q^*_o) $$ and $$ \xi(k^{sup}_I(q^*_o),q^*_o)=\sup_{q^*}\xi(k^{sup}_I(q^*),q^*)$$
If $ q^*_{stat,\kappa}=q^*_{stat,\iota} $, then $ q^*_o=q^*_{stat,\kappa}=q^*_{stat,\iota} $ and the results follow, so we assume $ q^*_{stat,\kappa}\neq q^*_{stat,\iota} $ ,then $$ \kappa_I(q^*)(q^*_{stat,\kappa})=\max_{q^*}\kappa_I(q^*)=\max_{q^*}\iota_I(q^*)>\iota_I(q^*)(q^*_{stat,\kappa}) $$ Similarly, $$ \iota_I(q^*)(q^*_{stat,\iota})>\kappa_I(q^*)(q^*_{stat,\iota}) $$ Then there exists $ q^*_o $ between $ q^*_{stat,\kappa} $ and $ q^*_{stat,\iota} $ such that $$ \kappa_I(q^*_o)=\iota_I(q^*_o) $$ Now we prove this $ \kappa_I(q^*_o)=\iota_I(q^*_o) $ is the maximum of $ \min\{\kappa_I(q^*),\iota_I(q^*)\} $: If there exists $ q^*_\pi\neq q^*_o $ such that both $ \kappa_I(q^*_\pi) $ and $ \iota_I(q^*_\pi) $ are greater than $ \kappa_I(q^*_o)=\iota_I(q^*_o) $, then if $ q^*_\pi>q^*_o $, $ q^*_\pi $ must be greater than one of the two stationary points which means one of $ \kappa_I(q^*),\iota_I(q^*) $ must decrease which is a contradiction since both $ \kappa_I(q^*_\pi) $ and $ \iota_I(q^*_\pi) $ are greater than $ \kappa_I(q^*_o)=\iota_I(q^*_o) $, similar analysis for $ q^*_\pi<q^*_o $. So we proved $$ \kappa_I(q^*_o)=\iota_I(q^*_o) $$ is the maximum of $ \min\{\kappa_I(q^*),\iota_I(q^*)\} $ given the properties of $ \{\kappa_I(q^*),\iota_I(q^*)\} $.

Now we begin to prove these properties and show that $$ NG(k^{sup}_I(q^*_{o}),q^*_{o})(0,1)=NG(k^{sup}_I(q^*_{o}),q^*_{o})(1,0)  $$


$ I = a $:\\
Based on Lemma~\ref{kvalue}, $ k^{sup}(q^*)=\frac{f(\tru\one)_y-f(\tru\zer)_y}{f(\tru\one)_x-f(\tru\zer)_x}=\frac{q(1|1) (1-q^*)}{q(0|0) q^*} $
\begin{align*}
\xi(k^{sup}_a(q^*),q^*)&=\phi^{k^{sup}_a(q^*),q^*}(k^{sup}_a(q^*))\\
&=\frac{q(1|0) (f(\tru\one)_x - f(\tru)_x)}{q(0|1)+q(1|0)}(k^{sup}_a(q^*)-\frac{q(0|1)}{q(0|0)})/(\max\{(1+\frac{ k^{sup}_a(q^*) q(1|0)}{q(0|1)}) q^*,\frac{ k^{sup}_a(q^*) q(1|0)}{q(0|1)} \})\\
&=\frac{q(1|0) (q^* - q(1|0))}{q(0|1)+q(1|0)}(k^{sup}_a(q^*)-\frac{q(0|1)}{q(0|0)})/(\max\{(1+\frac{ k^{sup}_a(q^*) q(1|0)}{q(0|1)}) q^*,\frac{ k^{sup}_a(q^*) q(1|0)}{q(0|1)} \})\\
&=\frac{1}{q(1|0)+q(0|1)}\min\{ \frac{q(1|0)q(0|1)(q(1|1)-q^*)(q^*-q(1|0))}{ q^*((q(1|1)-q(0|0))q^*-q(1|0)q(1|1)) },\frac{q(0|1)(q(1|1)-q^*)(q^*-q(1|0))}{q(1|1) (1-q^*)} \}
\end{align*}
Let $$ \kappa_a(q^*)=\frac{q(0|1)}{q(1|0)+q(0|1)}\frac{(q(1|1)-q^*)(q^*-q(1|0))}{q(1|1) (1-q^*)} $$ $$ \iota_a(q^*)=\frac{q(0|1)}{q(1|0)+q(0|1)} \frac{q(1|0)(q(1|1)-q^*)(q^*-q(1|0))}{ q^*((q(1|1)-q(0|0))q^*-q(1|0)q(1|1)) } $$ Then $$ \xi(k^{sup}_a(q^*),q^*)=\min\{ \kappa_a(q^*),\iota_a(q^*) \} $$ Notice that if $ \kappa_a(q^*_{a,o})=\iota_a(q^*_{a,o}) $ and $ q^*_{a,o}\neq q(1|0),q(1|1)  $, then $$ (1+\frac{ k^{sup}_a(q^*_{a,o}) q(1|0)}{q(0|1)}) q^*_{a,o}=\frac{ k^{sup}_a(q^*_{a,o}) q(1|0)}{q(0|1)} $$

\begin{align*}
\Rightarrow& NG(k^{sup}_I(q^*_{a,o}),q^*_{a,o})(0,0)-NG(k^{sup}_I(q^*_{a,o}),q^*_{a,o})(0,1)\\
=& NG(k^{sup}_I(q^*_{a,o}),q^*_{a,o})(0,0)-NG(k^{sup}_I(q^*_{a,o}),q^*_{a,o})(1,0)
\end{align*}
$$\Rightarrow  NG(k^{sup}_I(q^*_{a,o}),q^*_{a,o})(0,1)=NG(k^{sup}_I(q^*_{a,o}),q^*_{a,o})(1,0) $$
Now we will show
$$ \kappa_a(q(1|0) + q(1|1) - \frac{q(1|0) q(1|1)}{q^*})=\iota_a(q^*) $$ Once we show it, it's clear that $$ \max_{q^*}\kappa_a(q^*)=\max_{q^*}\iota_a(q^*) $$ when $ q(1|0)<q^*<q(1|1) $
\begin{align*}
\kappa_a(q(1|0) + q(1|1) - \frac{q(1|0) q(1|1)}{q^*})&=\frac{q(0|1)}{q(1|0)+q(0|1)}\frac{(\frac{q(1|0)q(1|1)}{q^*}-q(1|0))(q(1|1)-\frac{q(1|0)q(1|1)}{q^*})}{q(1|1) (q(0|0) - q(1|1) + \frac{q(1|0) q(1|1)}{q^*})}\\
&=\frac{q(0|1)}{q(1|0)+q(0|1)} \frac{q(1|0)(q(1|1)-q^*)(q^*-q(1|0))}{ q^*((q(1|1)-q(0|0))q^*-q(1|0)q(1|1)) }\\
&=\iota_a(q^*)\\
\end{align*}
Now we show that $ \kappa_a(q^*) $ is first increasing and then decreasing. Since $ \kappa_a(q(1|0))=\kappa_a(q(1|1))=0 $, $ \kappa_a(q^*)>0 $ when $ q(1|0)<q^*<q(1|1) $ and there are at most two stationary points of $ \kappa_a(q^*) $, so $ \kappa_a(q^*) $ must be first increasing and then decreasing. Since $ q(1|0) + q(1|1) - \frac{q(1|0) q(1|1)}{q^*} $ is a increasing function,  $ \iota_a(q^*) $ is also first increasing and then decreasing when $ q(1|0)\leq q^* \leq q(1|1) $.\\
We solve the equation $ \kappa_a(q^*)=\iota_a(q^*) $, except $ q^*=q(1|0),q(1|1) $, we also have two roots $$root_1=\frac{q(1|0) q(1|1)-\sqrt{(q(1|0)-1) q(1|0) (q(1|1)-1) q(1|1)}}{q(1|0)+q(1|1)-1}$$ $$root_2=\frac{q(1|0) q(1|1)+\sqrt{(q(1|0)-1) q(1|0) (q(1|1)-1) q(1|1)}}{q(1|0)+q(1|1)-1}$$
Since
\begin{align*}
root_2-q(1|1)&=\frac{\sqrt{(q(1|0)-1) q(1|0) (q(1|1)-1) q(1|1)}-q(1|1)^2+q(1|1)}{q(1|0)+q(1|1)-1}\\
&=\frac{\sqrt{q(1|1)q(0|1)}(\sqrt{q(1|1)q(0|1)}+\sqrt{q(1|0)q(0|0)})}{q(1|1)-q(0|0)}>0
\end{align*}
So $$ q^*_{a,o}=root_1 $$ after substitutions, we have

\begin{align*}
&\sup_{q^*}\xi(k^{sup}_a(q^*),q^*)=\\
&\frac{q(0|1)(q(0|0)q(1|0)-\sqrt{q(0|0)q(1|0)q(0|1)q(1|1)})(\sqrt{q(0|0)q(1|0)q(0|1)q(1|1)}-q(0|1)q(1|1))}{(q(0|1)+q(1|0)q(1|1)(q(1|1)-q(0|0))(\sqrt{q(0|0)q(1|0)q(0|1)q(1|1)}+q(1|1)-q(0|0)-q(1|0)q(1|1))} \end{align*}


let $ \Delta^*_a=\sup_{q^*}\xi(k^{sup}_a(q^*),q^*) $\\
and by the formula of $ NG(k,q^*) $ in Lemma~\ref{normpayoffkqstar} and subsititutions, we can also obtain $$NG(k^{sup}_a(q^*_{a,o}),q^*_{a,o})=\left( \begin{array}{ccc}
\zeta(Q) & & 0\\
 & & \\
0 & & 1\\
\end{array} \right)$$
where $  \zeta(Q)=\sqrt{\frac{q(0|0) q(0|1)}{q(1|0) q(1|1)}}   $

Since there is only one intersection point $ q^*_{a,o} $ of $ \kappa_{a}(q^*) $ and $ \iota_{a}(q^*) $, so when $ q^*_{a,o} \leq q^* $, one of $ \kappa_{a}(q^*) $ and $ \iota_{a}(q^*) $ must be less than another. Notice that we have
$$\kappa_a(q(1|0) + q(1|1) - \frac{q(1|0) q(1|1)}{q^*})=\iota_a(q^*)$$
and
\begin{align*}
q(1|0) + q(1|1) - \frac{q(1|0) q(1|1)}{q^*}-q^*=\frac{1}{q^*}(q(1|1)-q^*)(q^*-q(1|0))>0
\end{align*}
So $ \kappa_{a}(q^*)>\kappa_a(q(1|0) + q(1|1) - \frac{q(1|0) q(1|1)}{q^*})=\iota_{a}(q^*) $ when $ q^* $ is close to $ q(0|0) $ since $ \kappa_{a}(q^*) $ is decreasing now. Combining with the fact that when $ q^*_{a,o} \leq q^* $, one of $ \kappa_{a}(q^*) $ and $ \iota_{a}(q^*) $ must be less than another, we have $ \kappa_{a}(q^*)>\iota_{a}(q^*) $ when $ q^*_{a,o} \leq q^* $. So in $NG(k^{sup}_a(q^*),q^*)$, $$ \frac{1}{\alpha(k^{sup}_a(q^*),q^*)} = (1+\frac{ k^{sup}_a(q^*) q(1|0)}{q(0|1)}) q^* $$ when $ q^*_{a,o} \leq q^* $. When $ q(0|0)>q^*_{a,o} $, $ \epsilon>0 $, we use this property to calculate $$NG(k^{sup}_a(q(0|0)+\epsilon),q(0|0)+\epsilon)$$ and obtain  $$\left( \begin{array}{ccc}
\zeta(Q,\epsilon) & & \delta(Q,\epsilon)\\
 & & \\
0 & & 1\\
\end{array} \right) $$ where
$ \zeta(Q,\epsilon)=\frac{q(0|0) q(0|1)}{q(0|0) q(0|1) q(0|0)+\epsilon+q(1|0) (q(1|1)-q(1|1)
   q(0|0)+\epsilon)} $,\\
$ \delta(Q,\epsilon)=\frac{q(1|0) q(1|1) (q(0|0)+\epsilon-1)^2-q(0|0) q(0|1) q(0|0)+\epsilon^2}{q(0|0)+\epsilon (q(1|0)
      q(1|1) (q(0|0)+\epsilon-1)-q(0|0) q(0|1) q(0|0)+\epsilon)} $


I=b:\\
Based on Lemma~\ref{kvalue}, $ k^{sup}(q^*)=\frac{f(\tru\one)_y-f(\fal)_y}{f(\tru\one)_x-f(\fal)_x} $.
Like we did when $ I=a $, after all substitutions, we will get
\begin{align*}
\xi(k^{sup}_b(q^*),q^*)=\min\{\kappa_b(q^*),\iota_b(q^*) \} \\
\end{align*}
Where $$ \kappa_b(q^*)=\frac{q(0|1)(q(1|1)-q(0|0))}{q(1|0)+q(0|1)}\frac{(q^*-q(1|0))(q(0|0)-q^*)}{q(0|0)q(1|0)(q^*-q(0|1))} $$
$$ \iota_b(q^*)=\frac{q(0|1)(q(1|1)-q(0|0))}{q(1|0)+q(0|1)} \frac{(q^*-q(1|0))(q(0|0)-q^*)}{((q(0|0)q(1|0)+q(0|1)(q^*-1))(q^*-1)}$$
Replace $ q^* $ with $ \frac{q(0|0)q(1|0)}{1-q^*} $, we can prove $$ \kappa_b(\frac{q(0|0)q(1|0)}{1-q^*})=\iota_b(q^*) $$ then it's clear that $$ \max_{q^*}\kappa_b(q^*)=\max_{q^*}\iota_b(q^*) $$ when $ q(1|0)<q^*\leq q(0|0) $. Like we proved before when $ I=a $, we can also prove that both $ \kappa_b(q^*) $ and $ \iota_b(q^*) $ are first increasing and then decreasing when $ q(1|0)\leq q^*\leq q(0|0) $.\\
We solve the equation $ \kappa_b(q^*)=\iota_b(q^*) $, except $ q^*=q(0|0),q(1|1) $, we also have two roots
$$root_1=\frac{-q(1|0)^2-\sqrt{(q(1|0)-1) q(1|0) (q(1|0)-q(1|1))
   (q(1|0)+q(1|1)-1)}+q(1|0)+q(1|1)-1}{q(1|1)-1} $$
$$root_2=\frac{-q(1|0)^2+\sqrt{(q(1|0)-1) q(1|0) (q(1|0)-q(1|1))
   (q(1|0)+q(1|1)-1)}+q(1|0)+q(1|1)-1}{q(1|1)-1}$$
Since
\begin{align*}
root_2-q(1|0)&=-\frac{\sqrt{q(0|0) q(1|0) (q(1|1)-q(0|0)) (q(1|1)-q(1|0))}+q(0|0) (q(1|1)-q(0|0))}{q(0|1)}\\
&<0
\end{align*}
So $$q^*_{b,o}=root_1$$ after substitutions, we have $$ \Delta^*_b=\frac{(q(1|1)-q(0|0))(q(0|0)q(1|0)(q(1|1)-q(0|1))-\sqrt{q(0|0)q(1|0)(q(1|1)-q(1|0))(q(1|1)-q(0|0))})}{(q(1|0)+q(0|1))q(1|0)q(1|1)q(0|0)} $$ and
$$ NG(k^{sup}_b(q^*_{b,o}),q^*_{b,o})=\left( \begin{array}{ccc}
1 & & 0\\
 & & \\
0 & & \eta(Q)\\
\end{array} \right) $$
where $ \eta(Q)=\frac{1}{q(1|1)}(\sqrt{\frac{(q(1|1)-q(1|0))(q(1|1)-q(0|0))}{q(0|0)q(1|0)}}-q(0|1))   $
\end{proof}


%We are going to show that the gap function only depends $ k $ and $ q^* $ of a payoff function $ PF $ if $ PF\in\mathcal{U} $:


%\begin{definition}
%We define $ G(\alpha,-k \alpha\frac{q(1|0)}{q(0|1)},q^*,\gamma)=G(\alpha,-\frac{k \alpha q(1|0)}{q(0|1)},q^*,\gamma) $
%\end{definition}







\else
All formal statements and proofs for this section appear in the full version. In this section, we first show that the gap $ \Delta_Q(PF) $ we want to optimize over payoff functions with payoffs in $ [0,1] $ region only depends on $ q^* $ and $ k $ where $ q^* $ is the ``break even" point and $ k $ is the slope of contours in $ R_{\tru} $ region in the mechanism under payoff function $ PF $. Then we fix $ q^* $ and tune $ k $ to optimize the gap.  Typically, the way that the gap is maximized corresponds to setting $k$ (the slope of contours in $ R_{\tru} $ region) to equalize the expected payments of the two equilibrium which correspond to adjacent extremal points to $\tru$ on the convex hull $\mathcal{H}$ of informative equilibrium translated into the $R_{\tru}$ quadrant of the best-response plot.  When $q^* > q(0|0)$ this this corresponds to making $\tru\one$ and $\tru\zer$ pay the same, and when $q^* < q(0|0)$ this this corresponds to making $\tru\one$ and $\fal$ pay the same.


After we finish that, the gap function will only be a function of $ q^* $ and at that time we will optimize the gap over $ q^* $.  The interesting part here is that there may be a discontinuity at $q^* = q(0|0)$.  If the optimum occurs when $q^* > q(0|0)$, then we are in $R_1$.  If the optimum occurs when $q^* < q(0|0)$, then we are in $R_2$.  If the optimum occurs at the boundary, then we are in $R_3$, and this accounts for the ``unattainable" region.  In the end, we use the best $ k,q^* $ to construct the mechanisms in Theorem~\ref{opt_thm}.



\fi





==> peer-eq-analysis.tex <==
%\jz{We should add the proof for assymetric equilibria in this section}
%
%In this section we discuss the problem of multiple equilibria in Peer Prediction games instantiated with strict proper scoring rules when $\Sigma = \{0, 1\}$.   We show that there are between 7 and 9 symmetric Bayesian Nash Equilibria in these mechanisms. We will assume that $Q$ is symmetric and that the bits are informative and positively correlated, i.e.\ $q(b | \neg b) < q(b|b)$.   If the bits of $Q$ are independent, then each user has no information about the others and peer-prediction will fail.  If the bits are negatively correlated, a similar analysis goes through, but we do not provide it here.
%
%Recall that $q^*(1)$ is such that $$PS(q^*(1), q(1|\hat{b}_i)) = PS(q^*(1), q(1|\neg \hat{b}_i)).$$   By Claim~\ref{claim:qstar} we know that $q(1|0) < q^*(1) < q(1|1)$.
%
%\begin{theorem}
%Let $Q$ be a symmetric, informative, and positively correlated prior on $\{0, 1\}^n$, and let $\mathcal{M}$ be a peer-prediction mechanism run with a strictly proper scoring rule with break-even $q^*(1)$. Then the symmetric equilibria are
% $$\zer, \one, \top, \strat{q^*(1)}{q^*(1)}, \strat{0}{\frac{q^*(1)}{q(1|1)}},\strat{\frac{q^*(1)-q(1|0)}{q(0|0)}}{1}$$
% and also conditionally include
%\begin{eqnarray}
%\fal & & \mbox{if } q(0|1) \leq q^*(1) \leq  q(0|0) \label{eq:always-lie} \\
%\strat{1}{\frac{q^*(1)-q(0|1)}{q(1|1)}} & & \mbox{if } q(0|1) \leq q^*(1)   \label{eq:zero-lie-one-amb} \\
%\strat{\frac{q^*(1)}{q(0|0)}}{0} & & \mbox{if }  q^*(1) \leq q(0|0)  \label{eq:one-lie-zero-amb}
%\end{eqnarray}
%\end{theorem}
%
%Because either the conditions of Equation~\ref{eq:zero-lie-one-amb} or of Equation \ref{eq:one-lie-zero-amb} are satisfied, there are always between 7 and 9 equilibria.   Additionally, we note that if the conditions of Equation~\ref{eq:zero-lie-one-amb} or \ref{eq:one-lie-zero-amb} are equalities, then the corresponding equilibrium is equivalent to the $\fal$ equilibrium.
%
%%\begin{wrapfigure}{ru}{.5\textwidth}
%%  % \fbox{
%%    \begin{minipage}{.5\textwidth}
%%    \vspace{-1.1\baselineskip}
%%  \begin{center}
%%    \includegraphics[width=\textwidth]{plot-of-equilibrium.png}
%%  \end{center}
%%  \vspace{-2\baselineskip}
%%  \caption{Equilibrium for Example~\ref{example}.} \label{fig:plot-of-equilibrium}
%%  \vspace{-1\baselineskip}
%%  \end{minipage}
%%\end{wrapfigure}
%
%
%\begin{figure}[htbp]
%\begin{center}
%\includegraphics[scale=.5]{plot-of-equilibrium.png}
%\caption{Equilibria for Example~\ref{example}. \label{fig:plot-of-equilibrium}}
%\vspace{-2\baselineskip}
%\end{center}
%\vspace{\baselineskip}
%\end{figure}
%
%
%Figure~\ref{fig:plot-of-equilibrium} shows the 7 equilibria that exist in Example~\ref{example} using the Brier scoring rule, which are $\zer, \one, \top,$
% \begin{align*}
%    \strat{q^*(1)}{q^*(1)} &\approx \strat{.594}{.594}, \\
%  \strat{0}{\frac{q^*(1)}{q(1|1)}}&\approx \strat{0}{.955},\\
%  \strat{\frac{q^*(1)-q(1|0)}{q(0|0)}}{1}&\approx \strat{.064}{1},\mbox{ and}\\
%   \strat{1}{\frac{q^*(1) - q(0|1)}{q(1|1)}}&\approx \strat{1}{.348}.
%  \end{align*}
% Note that to the right of the red line where $\hat{q}(1|0) = q^*(1)$, the best response is to increase $\theta(1|0)$; to the left of the red line, the best response is to decrease $\theta(1|0)$; and on the line an agent is indifferent.    Similarly, above the blue line where $\hat{q}(1|1) = q^*(1)$, the best response is to increase $\theta(1|1)$; below the blue line, the best response is to decrease $\theta(1|1)$; and on the line an agent is indifferent.
%
%If Example~\ref{example} were such that $q^*(1)$ were closer to $1/2$, then the red line would intersect the bottom half of the square and there would be two additional equilibria, one at $\bot$ and the other at the intersection.  Exactly 8 equilibria would exist if the intersection of the red line with the edges of the square were exactly at $\bot$.
%

%\gs{This should (I hope) go away at some point}\jz{We still need this claim in the preliminaries to explain the best responses in the contour plots of section 4}
%
%\begin{claim}\label{claim:equil-crit}
%Given $q^*(1), q(1|0), q(1|1)$, a profile $\theta$ is an equilibrium of a peer prediction mechanism for binary signals if and only if:
%\begin{itemize}
%\item if $\theta(1|b) > 0$, then $\hat{q}(1|b) \geq q^*(1)$
%\item if $\theta(1|b) < 1$, then $\hat{q}(1|b) \leq q^*(1)$
%\end{itemize}
%\end{claim}
%
%\begin{proof}
%First, we show that the conditions are necessary by the contrapositive: If $\hat{q}(1|b) < q^*(1)$ then for $\theta$ to be an equilibrium, we must have $\theta(1|b) = 0$.  This follows from the definition of $q^*(1)$.  Similarly, if $\hat{q}(1|b) > q^*(1)$  then  for $\theta$ to be an equilibrium, we have $\theta(1|b) = 1$.
%
%Next, assuming $\theta$ satisfies both conditions,  we can show it is an equilibrium.  Assume an agent receives a bit $b$.  Then if $\theta(1|b) \not \in \{0, 1\}$, $\hat{q}(1|b) = q^*(1)$, thus the agent is indifferent between playing 0 and 1.  If $\theta(1|b) = 0$, then $\hat{q}(1|b) \leq q^*(1)$, and so playing 0 is at least as good as playing 1.  Similarly if $\theta(1|b) =1$, then $\hat{q}(1|b) \geq q^*(1)$ and so playing 1 is at least as good as playing 0.
%\end{proof}

\begin{comment}
We analyze all possible equilibria by looking at four possible cases:.
\begin{itemize}
\item  $\theta(1|0) \in \{0, 1\}$ and $\theta(1|1) \in \{0, 1\}$;
\item  $\theta(1|0) \in \{0, 1\}$ but $\theta(1|1) \not\in \{0, 1\}$;
\item  $\theta(1|0) \not\in \{0, 1\}$ but $\theta(1|1) \in \{0, 1\}$;
\item  $\theta(1|0) \not\in \{0, 1\}$ and $\theta(1|1) \not\in \{0, 1\}$.
\end{itemize}

We consider each case in turn.




\paragraph* {Both $\theta(1|0)$ and $\theta(1|1)$ are integral}  This means that the agents are all playing the same pure-strategy in $S$.  There are four possibilities:
\begin{description}
\item[$\zer$, everyone reports 0]

This equilibrium always exists.

Intuitively, this is an equilibrium because if everyone reports 0, then predicting 1 is not a good strategy.

Formally, this is an equilibrium by Claim~\ref{claim:equil-crit} because $\theta(1|0)= 0 < 1$ and $\hat{q}(1|0) \leq q^*(1)$, similarly $\theta(1|1)= 0 < 1$ and $\hat{q}(1|1) = 0 \leq q^*(1)$.

\item[$\one$, everyone reports 1]

This equilibrium always exists.

Intuitively, this is an equilibrium because if everyone reports 1, then predicting 0 is not a good strategy.

Formally, this is an equilibrium by Claim~\ref{claim:equil-crit} because $\theta(1|1)= 1 > 0$ and $\hat{q}(1|1) \geq q^*(1)$, similarly $\theta(1|0)= 1 > 0$ and $\hat{q}(1|1) = 1 \geq q^*(1)$.  %This is analogous to the case were everyone plays 0.

\item[$\tru$, everyone reports the truth]

This equilibrium always exists.

 We know this is an equilibrium from properties of the proper scoring rule.

 Formally, this is an equilibrium by Claim~\ref{claim:equil-crit}.  $\theta(1|0) = 0 < 1$ so we must check that $\hat{q}(1|0) \leq q^*(1)$  However, $\hat{q}(1|0) = q(1|0) <  q^*(1)$.  Additionally, $\theta(1|1) = 1 > 0$ so we must check that $\hat{q}(1|1) \geq q^*(1)$.  However, $\hat{q}(1|1) = q(1|1) >  q^*(1)$.

\item[$\bot$, everyone lies]
This is an equilibrium if and only if $q(0|1) \leq q^*(1) \leq q(0|0) $. This equilibrium need not exist.

 Intuitively, the conditions for existence will hold if $q^*(1)$ is close to 1/2.  If the prior is symmetric about 0 and 1, then this will be an equilibrium because the mechanism has no way of differentiating between 0 and 1 which are merely swapped.  However, if the prior is severely skewed, then this will not be an equilibrium.  Intuitively, if a player actually receives a rare type, he will want to exploit that the common types are also playing it.

 Formally, again employing Claim~\ref{claim:equil-crit}, $\theta(1|0) = 1 > 0$ so we must check that $\hat{q}(1|0) \geq q^*(1)$.  However, $\hat{q}(1|0) = q(0|0) \geq q^*(1)$ (by assumption).  Additionally, $\theta(1|1) = 0 < 1$ so we must check that $\hat{q}(1|1) \leq q^*(1)$.  However, $\hat{q}(1|1) = q(0|1) \leq q^*(1)$.
    If, for example, $q^*(1)$, $q(1 | 1)$ and $q(0 | 1)$ are all less then 1/2, then a player seeing a 1 is better off playing a 1 (the truth), because $\hat{q}(1|0) = q(0|0) = 1 - q(1|0) > 1/2 > q^*(1)$.
\end{description}

\paragraph*{$\theta(1|0) \in \{0, 1\}$ but $\theta(1|1) \not\in \{0, 1\}$;}

There are two possibilities:

\begin{description}
\item[$\strat{0}{\theta(1|1)}$, players receiving 0 always tell the truth  and players receiving 1 sometimes lie]

 This is an equilibrium if and only if $\theta(1|1) = \frac{q^*(1)}{q(1|1)}$. This equilibrium always exists.

First we note by Claim~\ref{claim:equil-crit} that for this to be an equilibrium we must have $\hat{q}(1|1) = q^*(1)$ because $0 < \theta(1|1) < 1$.
Setting $\hat{q}(1|1) = q^*(1)$ and $\theta(1|0) = 0$ in Equation~\ref{eqn:p1} we get $q^*(1) = \theta(1|1) q(1|1) \Rightarrow \theta(1|1) = \frac{q^*(1)}{q(1|1)}$.
By the assumption that the proper scoring rule is strict and the signals are positively correlated, we know that the value of $q^*(1)$ is unique and induces a unique non-integral value of $\theta(1|1)$, and such a value exists. %Because $q^*(1) < q(1|1)$ this is between 0 and 1.  Thus there is at most one such equilibrium.
To verify this is an equilibrium, we again use Claim~\ref{claim:equil-crit}.  We see that $\theta(1|0) = 0 < 1$ and so must check that $\hat{q}(1|0) \leq q^*(1)$.  However, $\hat{q}(1|0) =  \theta(1|0) q(0|0)  + \theta(1|1) q(1|0) = 0 + \frac{q^*(1)}{q(1|1)}q(1|0) \leq q^*(1)$ because $q(1|0) \leq q(1|1)$, by the assumption that the prior is positively correlated.

\item[$\strat{1}{\theta(1|1)}$, players receiving 0 always lie and players receiving 1 sometimes lie]  This is an equilibrium iff $q(0|1) < q^*(1)$ and $\theta(1|1)= \frac{q^*(1) - q(0|1)}{q(1|1)}$. This equilibrium need not exist.


First we note that by Claim~\ref{claim:equil-crit} for this to be an equilibrium we must have $\hat{q}(1|1) =  q^*(1)$ because $0 < \theta(1|1) < 1$.  Setting $\hat{q}(1|1) = q^*(1)$ and $\theta(1|0) = 1$ in Equation~\ref{eqn:p1} we get $q^*(1) = q(0|1) + \theta(1|1)q(1|1) \Rightarrow \theta(1|1) = \frac{q^*(1) - q(0|1)}{q(1|1)}$.  This is less than 1 because $q^*(1) < q(1|1)$, by the assumptions of the strictness of the proper scoring rule and the positive correlation of the signals.  This is greater than 0 only if  $q(0|1) < q^*(1)$.  Thus there is at most one such equilibrium in this situation and none otherwise.  To verify this is an equilibrium when  $q(0|1) < q^*(1)$, we see that $\theta(1|0) = 1 > 0$ and so must check that $\hat{q}(1|0) \geq  q^*(1)$.  However,
\begin{align*}
\hat{q}(1|0) = & \theta(1|0)q(0|0) + \theta(1|1)q(1|0) \\
             = & q(0|0) + \frac{q^*(1) - q(0|1)}{q(1|1)}q(1|0) \\
             = & 1 - q(1|0) + \frac{q^*(1) - 1 + q(1|1)}{q(1|1)}q(1|0) \\
             = & \frac{q(1|0)}{q(1|1)}q^*(1)  + \frac{q(1|1) - q(1|0)}{q(1|1)} \\
             > & \left(\frac{q(1|0)}{q(1|1)} + \frac{q(1|1) - q(1|0)}{q(1|1)}\right)q^*(1) \\
             = & q^*(1)
\end{align*}
\end{description}

\paragraph*{$\theta(1|1) \in \{0, 1\}$ but $\theta(1|0) \not\in \{0, 1\}$;}

There are two possibilities:

\begin{description}

\item[$\strat{\theta(1|0)}{1}$, players receiving 1 always tell the truth  and players receiving 0 sometimes lie]   This is an equilibrium if $\theta(1|0) = \frac{q^*(1) - q(1|0)}{q(0|0)}$.  This equilibrium always exists.

This is analogous to the case where players receiving 0 always tell the truth  and players receiving 1 sometimes lie, and the result follows by the above analysis by simply switching the labels 0 and 1.  Before we showed that $\theta(1|1) = \frac{q^*(1)}{q(1|1)}$.  Switching the labels gives us:
$$\theta(0|0) = \frac{q^*(0)}{q(0|0)} \Rightarrow \theta(1|0) = 1 -  \frac{1 - q^*(1)}{q(0|0)} = \frac{q^*(1) - q(1|0)}{q(0|0)}$$ which is what we sought.

\item[$\strat{\theta(1|0)}{0}$, players receiving 1 always lie and players receiving 0 sometimes lie]  This is an equilibrium if $q^*(1) < q(0|0)$ and $\theta(1|0) = \frac{q^*(1)}{q(0|0)}$.  This equilibrium need not exist.

 This is analogous to the case where players receiving 0 always lie and players receiving 1 sometimes lie, and the result follows by the above analysis by simply switching the labels 0 and 1.  In the previous case, we showed that this is an equilibrium when $q(0|1) < q^*(1)$ and  $\theta(1|1) = \frac{q^*(1) - q(0|1)}{q(1|1)}$.  Switching the labels gives us that this is an equilibrium when $q(1|0) < 1 - q^*(1) \Rightarrow q^*(1) < q(0|0)$ and
      $$\theta(0|0) = \frac{q^*(0) - q(1|0)}{q(0|0)}\Rightarrow \theta(1|0) = 1 - \frac{1 - q^*(1) - q(1|0)}{q(0|0)} =  \frac{q^*(1)}{q(0|0)}$$
\end{description}


\paragraph*{Neither $\theta(1|0)$ nor $\theta(1|1)$ is integral.}
This is an equilibrium if $\theta(1|1) = \theta(1|0) = q^*(1)$. This equilibrium always exists.


By Claim~\ref{claim:qstar}, it must be that $\hat{q}(1|1) = \hat{q}(1|0) = q^*(1)$.  Subtracting Equation~\ref{eqn:p1} from Equation~\ref{eqn:p0}  we have
\begin{align*}
0 = & \hat{q}(1|0) - \hat{q}(1|1) \\
  = & \theta(1|0)q(0|0) + \theta(1|1)q(1|0) - \theta(1|0)q(0|1) - \theta(1|1) q(1|1) \\
  = & \theta(1|0)(1 - q(1|0)) + \theta(1|1) q(1|0) - \theta (1|0)(1-q(1|1)) - \theta(1|1)q(1|1) \\
  = & \theta(1|0)(q(1|1) - q(1|0)) + \theta(1|1)(q(1|0)-q(1|1)) \\
  = & (\theta(1|0) - \theta(1|1))(q(1|1) - q(1|0))
\end{align*}
By the assumption that the prior is positively correlated, $q(1|1) > q(1|0)$, and so we conclude that $\theta(1|0) = \theta(1|1)$.

Now, adding Equation~\ref{eqn:p1} to Equation~\ref{eqn:p0}, we get that
\begin{align*}
2 q^*(1) = & \hat{q}(1|0) + \hat{q}(1|1) \\
  = & \theta(1|1)(q(0|0) + q(1|0) + q(0|1)+ q(1|1)) \\
  = & 2 \theta(1|1).
\end{align*}
Thus, we see that $\theta(1|1) = \theta(1|0) = q^*(1)$.
\vspace{10pt}

Because the four cases we analyzed exhaustively partition the space of possible symmetric Bayesian Nash equilibrium, there cannot be any other equilibria.

Summing up, we see that if $1 - q_0 < q^*(1) < 1 - q_1$ then there are 9 equilibria.  If either $1 - q_0 = q^*(1)$ or  $1 - q_1 = q^*(1)$ there are 8 equilibria.  Otherwise, if $1 - q_0 = q^*(1) = 1 - q_1$, there are 7 equilibria.
\end{comment}



%\katrina{Need to make clear why there can't be any other equilibria.}




==> zero-one_elimination.tex <==
In this section, we make $\tru$ focal when taking every equilibrium, including  $ \zer $ and $ \one$, into account. The idea is that we can eliminate the  $ \zer $ and $ \one $ equilibria by punishing all zero and all one reports with a large enough penalty. Such a penalty should only depend on other players' reports so as not to affect the set of equilibria.  We therefore an agent of all the \emph{other} agents report the same signal.  

There is a possible issue with this approach:  it might be the case that all players receive the same signal and that the truthful equilibrium will be penalized. Under certain conditions, this penalty will affect any informative equilibrium with low probability.  This the punishments expected impact informative equilibria will be overcome by the advantage of the truth-telling equilibrium's payments that we constructed in the previous section. On the other hand, the $\zer$ and $\one$ equilibria will fully bear this punishment, and hence have lower payoff than truth-telling.


\begin{claim}\label{shift}
Adding an arbitrary function of the other players' reports to the player payments does not
change the set of equilibria.
\end{claim}

\begin{proof}
It is well known that adding a term to agent $i$'s payoff that is only based on the actions of the other agents does not alter the set of equilibrium because the marginal gains/losses from unilateral deviation remain unchanged.
\end{proof}

We will use Claim~\ref{shift} to prove that we can make truthtelling focal among both informative and non-informative equilibria of the game by adding a function of the other players' reports to the payment of each player.
 
 

\begin{theorem} 
Let $Q$ be a binary symmetric prior such that $q(0|1) \neq q(1|0))$.  Let $\epsilon_Q$ be the maximum probably that a fixed set of $n-1$ agents receive the same signal (either all $\zer$ or all $\one$).  If $Q$ is attainable, let $PS^*$ be such that $\Delta_Q(PS^*) = \Delta^*(Q)$ and let $t = \nu^{PS^*}(\tru)$.  Otherwise let $\lim\sup_{\epsilon \rightarrow 0^+} \Delta_Q(PS^*(\epsilon)) = \Delta^*(Q)$  and let $t = \lim\sup_{\epsilon \rightarrow 0^+} \nu^{PS^*(\epsilon)}(\tru)$.
If $\epsilon < \frac{\Delta^*(Q)}{1 - t +\Delta^*(Q)}$  then there is a mechanism that makes truth-telling focal.
\end{theorem}

Note that once truth telling is focal, we can renormalized so that payments are between 0 and 1.  In particular, this theorem says that if $\epsilon_{Q} \rightarrow 0$ (say as the number of agents increases), then at some point, truthtelling will be focal.  We know that such a limit is necessary because, for example, with two agents making truthtelling focal is impossible.  \gs{add citation}

\begin{proof}
We will design a mechanism $\bar{PS}^*$ identical to $PS*$ (or $\bar{PS}^*(\epsilon)$) except that we will issue a punishment of $ p = \frac{1-t}{2(1-\epsilon_Q)} + \frac{\Delta^*(Q)}{2 \epsilon_Q}$ to an agent if all the other agents play all $\zer$ or all $\one$.

By our assumption on $\epsilon_Q$, we know that $\frac{1-t}{1-\epsilon_Q} < \frac{\Delta^*(Q)}{ \epsilon_Q}$ .  Because $p$ is the average of these two values, we have $\frac{1-t}{1-\epsilon_Q} < p < \frac{\Delta^*(Q)}{ \epsilon_Q}$.

By Claim~\ref{shift} the equilibrium of $\bar{PS}^*$ (or $\bar{PS}^*(\epsilon)$) are the same as those of ${PS}^*$ (or ${PS}^*(\epsilon)$).

On the one hand, the expected payment of truthtelling has decrease by at most $\epsilon_Q p$ because in the truthtelling equilibrium, all agents report there true signals, and for any set of $n-1$ agents, all these signals are identical with probability at most $\epsilon_Q$.  However, $\epsilon_Q p < \Delta^*(Q)$.  If $Q$ is unattainable let $\epsilon  =  \frac{ \Delta^*(Q) - \epsilon_Q}{2}$.  Then the payment for truth-telling in $\bar{PS}^*$ (or $\bar{PS}^*(\epsilon)$  is still greater than the payment for any other non-informative equilibrium (note that the payments for all equilibria only decreased).


On the other hand, the payment for the all zero or one equilibrium is now at most $1 - p = 1 - (p - \epsilon_Q p) - \epsilon_Q p  < 1 - (1- t) - \epsilon_Q p =  t - \epsilon_Q p$.   And so truthtelling now pays more than the all 0 or all 1 equilibria.
\end{proof}

 



